Towards Linguistic Neural Representation Learning and Sentence Retrieval from Electroencephalogram Recordings

Decoding linguistic information from non-invasive brain signals using EEG has gained increasing research attention due to its vast applicational potential. Recently, a number of works have adopted a generative-based framework to decode electroencephalogram (EEG) signals into sentences by utilizing the power generative capacity of pretrained large language models (LLMs). However, this approach has several drawbacks that hinder the further development of linguistic applications for brain-computer interfaces (BCIs). Specifically, the ability of the EEG encoder to learn semantic information from EEG data remains questionable, and the LLM decoder's tendency to generate sentences based on its training memory can be hard to avoid. These issues necessitate a novel approach for converting EEG signals into sentences. In this paper, we propose a novel two-step pipeline that addresses these limitations and enhances the validity of linguistic EEG decoding research. We first confirm that word-level semantic information can be learned from EEG data recorded during natural reading by training a Conformer encoder via a masked contrastive objective for word-level classification. To achieve sentence decoding results, we employ a training-free retrieval method to retrieve sentences based on the predictions from the EEG encoder. Extensive experiments and ablation studies were conducted in this paper for a comprehensive evaluation of the proposed approach. Visualization of the top prediction candidates reveals that our model effectively groups EEG segments into semantic categories with similar meanings, thereby validating its ability to learn patterns from unspoken EEG recordings. Despite the exploratory nature of this work, these results suggest that our method holds promise for providing more reliable solutions for converting EEG signals into text.

==> relatedworks.tex <==
The brain-to-text decoding field has evolved rapidly, starting with Anumanchipalli et al.'s 2019 breakthrough in decoding ECoG signals into speech waveforms \cite{anumanchipalli_2019_speech_synthesis_neural_spoken_sentences_ecog_bilstm_brain2speech}. This was followed by innovative uses of GANs by Wang et al. in 2020 \cite{wang_2020_stimulus_speech_ecog_decoding_cortex_gan_brain2speech}, and the application of RNNs and language models for text decoding from neural signals during handwriting by Willett et al. in 2021 \cite{Willett_2021_ecog_brain2text_handwriting_rnn_lm_brain2text}. Further advancements included real-time decoding of speech and text by Metzger et al. in 2023 \cite{Metzger_2023_ecog_hubert_birnn_brain2speech_brain2text_avatar}, and the decoding of logosyllabic languages into pinyin by Liu et al. \cite{Liu_2023_ecog_chinese_cnn_lstm_brain2speech_brain2pinyin}.

Non-invasive methods have also seen progress, albeit more limited in scope. Meta's use of contrastive learning with MEG and EEG signals for brain-to-speech decoding \cite{D_fossez_2023_meg_eeg_clip_pretrain_meta_brain2speech} and Wang et al.'s work on EEG-based text decoding \cite{wang2022open_aaai_eeg2text} stand out, though they lack the capability for open-vocabulary decoding. DeWave~\cite{duan2023dewave} introduce discrete codex into brain encoding, and BELT~\cite{zhou2023belt,chau2023belt} further introduces contrastive learning to enhance the coding quality. NuSpeech~\cite{yang2024decode} propose to utilize end-to-end speech decoding model Whisper~\cite{radford2023robust} and reach good performance. However, these end-to-end models encounter the same issue: possessing a powerful decoder does not necessarily incentivize the encoder to better learn the brain's dynamic features. Conversely, a stronger decoder may lead to a situation where the decoder, in a rather cunning manner, memorizes all test sentences without genuinely understanding or processing them.

This work takes a step back, deconstructing the decoding process into two stages with the aim to first ensure that the encoder learns adequate features. Subsequently, the real decoding capability is measured using an unbiased decoder, one that is not obtained through training.


==> test.tex <==
duan2023dewave_brain2text
